Facilitating SQL Query Composition and Analysis

Formulating efficient SQL queries requires several cycles of tuning and execution, particularly for inexperienced users. We examine methods that can accelerate and improve this interaction by providing insights about SQL queries prior to execution. We achieve this by predicting properties such as the query answer size, its run-time, and error class. Unlike existing approaches, our approach does not rely on any statistics from the database instance or query execution plans. This is particularly important in settings with limited access to the database instance. Our approach is based on using data-driven machine learning techniques that rely on large query workloads to model SQL queries and their properties. We evaluate the utility of neural network models and traditional machine learning models. We use two real-world query workloads: the Sloan Digital Sky Survey (SDSS) and the SQLShare query workload. Empirical results show that the neural network models are more accurate in predicting the query error class, achieving a higher F-measure on classes with fewer samples as well as performing better on other problems such as run-time and answer size prediction. These results are encouraging and confirm that SQL query workloads and data-driven machine learning methods can be leveraged to facilitate query composition and analysis.

==> Background-v2.tex <==


\section{Background: Models}
\label{appendix:dbrec-models}

 
In the following, we first provide an overview of general NLP modeling methods for constructing vectors from textual data. 
Let $\mathcal{Q}$ denote the collection of all queries, where each query  is a set of $n$ tokens, $Q = \{t_i\}_{i=1}^n$.    The goal of all models  is to map each query to a  vector $\bm{h} \in \mathbb{R}^k$.

%\subsubsection{General NLP Modeling Approaches}
\subsection{Overview}
\label{subsec:dbrec_vector_rep}

Similar to   natural language, SQL queries  have a compositional structure where smaller units are combined to create larger units. In particular characters are combined into  tokens, which are  combined into longer constructs, like  lines and blocks of code. 
This compositional structure imposes  the following considerations for generating vector representations:

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\vspace{4mm}\noindent \textbf{Model granularity level. } The  level of granularity of the input data that the model considers  determines the smallest unit of input, which we refer to as \textit{tokens}. Common granularity levels are   character-level and word-level.
 %(i.e., consider each word as an atomic item)   %(i.e., consider each character as an atomic item)
 For example, the query  in Figure~\ref{dbrec:fig_Q1} has 48 tokens at  the character level (excluding spaces), and  8 tokens at the word-level. %, 55 characters (with spaces). 
 In text applications,  n-gram granularity level can also be considered.  An n-gram is a sequence of $n$ tokens  that appear in the document. For example a 3-gram considers sequences of length 3 as tokens. The domain \textit{vocabulary}  is the set of all possible tokens.
Word-level models are commonly used in NLP tasks.   To prevent the vocabulary from getting too large,   rare tokens and digits are  removed,    and  out-of-vocabulary (OOV) words  are replaced with an unknown token,  $<$UNK$>$~\cite{zolaktaf2011modeling}. %Digits can also be removed, or replaced  with a token <DIGIT>. 
 When there are many  rare or OOV tokens in a domain, character-level models can instead be used. Although they result in longer input sequences,   they can  provide a boost in accuracy~\cite{kim2016character,zhang2015character}.

  %, i.e., a document of $n$ words, can have $n * 10$ characters on average, 


\vspace{4mm}\noindent \textbf{Token representation. }  Two alternatives are \textit{symbolic} and \textit{distributed} representations. 
In  symbolic representations, each token  is represented by one symbol or feature. %single atomic unit
Let $V$ denote the size of the domain vocabulary. In vector space terms, each   token  is associated with an index $j$ in a  $V$-dimensional binary vector $\bm{e} \in \{0,1\}^V$,  where element $j$ is equal to 1, and the remaining elements are zero.    This is also called the  \textit{one-hot} encoding scheme.
But this  representation  does not define an inherent notion of  meaning  for  tokens. %For example, computing  the dot product between the one-hot vectors  of different queries is always zero.
% Deep learning frameworks use large-scale corpora to learn real-valued vector representations  for words, referred to as \textit{distributed representations}.  

In  distributed representations,  each token is represented by many features. In particular, the meaning of each token  is encoded by  a real-valued d-dimensional vector $\bm{x} \in \mathbb{R}^d$.  These vectors can be based on co-occurrence statistics in the corpora. Deep learning frameworks can use large-scale corpora to learn the  semantic and syntactic aspects of the corpora in these representations~\cite{mikolov2013distributed}. 


%Finally, for longer constructs such as sentences, the tokens must be combined into a global vector~\cite{li2015tree}. longer constructs
\vspace{4mm}\noindent \textbf{Combining tokens  into global vectors. }  Traditional models used the bag-of-words (BOW) model to combine   symbolic representations into a global vector that represents longer constructs, like sentences.  In BOW, token order is not considered. For example,  a simple BOW representation is the sum  of  one-hot encoding vectors of words. 
For distributed representations, in addition to  BOW, sequence and tree-structured models are commonly used~\cite{tai2015improved,li2015tree}. %An example of  BOW model is  the average over the  distributed representations of individual tokens. 
Sequence models consider token order. They process and combine the tokens sequentially to obtain the global vector. %The only linguistic structure they consider is the word order. 
Examples include standard Recurrent Neural Networks (RNN), which we explore in Section~\ref{subsec:dbrec-3layerlstm}.
Tree-structured models  process and combine the words according to a tree order, bottom-up until they reach the root.  %So, the linguistic structure they consider is the parse tree. 
Examples include standard recursive models %referred to as Tree-RNN in~\cite{tai2015improved}  
or Tree-LSTM models~\cite{tai2015improved}.  RNNs are also regarded as a simple recursive model that processes words from left to right~\cite{conneau2016very}.   

\subsection{Bag-of-ngrams and its TFIDF}
\label{subsec:dbrec-ngram_TFIDF}
This model  uses n-gram tokens, with symbolic  representations, and combines them according to the BOW model. We explain the details in the context of SQL queries. %$q \in \mathbb{R}^{|V|}$
Each query  is a set of  tokens, $q = \{q_t\}_{t=1}^{|q|}$.  Let $\mathcal{Q}$ denote the collection of all queries, and $V$ denote the size of the  domain vocabulary. 
In the TFIDF   vector representation, each query is represented by a $V$-dimensional  vector. The weight of a token  $q_t$   is computed using   \begin{align*}
TFIDF (q_t, q, \mathcal{Q}) = TF( q_t,q) . IDF( q_t,\mathcal{Q})
\end{align*}
where $TF(q_t,q)$ is the normalized  frequency of term $q_t$  in  query $q$. The normalization  prevents bias towards longer queries.
The $IDF(q_t,\mathcal{Q})$  component describes the discriminative power of  term  $q_t$ in  the entire  collection of queries $\mathcal{Q}$, and helps to control for the fact that some terms are generally more common than other terms. It can be computed by $\log{\frac{|\mathcal{Q}|}{ 1 +|\{q \in \mathcal{Q} : q_t \in q\}|}}$, where the denominator is  the number of queries in the collection that contain term $q_t$.   The TFIDF value increases proportionally to the frequency of a  term in a document, but is counterbalanced by the frequency of the term in the collection. The logarithm function in the IDF term component helps to scale the ratio into a smaller range of $[0,1]$.  As a term appears in more documents, the ratio inside the logarithm approaches 1, bringing the IDF and TFIDF closer to 0. 


\subsection{RNN}
\label{subsec:dbrec-lstm}

\begin{figure}[t]
\centering
	\iffullpaperComposition
       \includegraphics[width=0.75\textwidth]{architecture/zrnn5}
	\else
	 \includegraphics[width=0.7\linewidth]{architecture/zrnn5}
	\fi
\caption{An example RNN network with hidden-to-hidden recurrent connections.  The RNN has a repetitive structure. The left hand side,   the recurrent graph is shown, while it is  unfolded on the right. At every time step $t$, the embedding $\bm{x}_t$ of a token in the sequence is  fed into the RNN. %The resulting hidden state $\bm{h}_t$ can be used to produce a label for classification problems.  
} 
\label{fig:rnn} 
\end{figure}

Recurrent Neural Networks (RNN) can process varying length input sequences such as  characters  or word tokens in a SQL query.
Figure~\ref{fig:rnn} shows a standard  RNN network. % RNNs read the input sequence, one token at a time, and construct a large fixed-dimensional vector representation. We
 Let $\bm{e}_t$ denote the one-hot encoding  of token $q_t$, and $\bm{X} \in \mathbb{R}^{d \times V}$ denote the embedding matrix. The distributed representation or embedding of term $q_t$   is obtained by a simple look up $\bm{x}_t = \bm{X}\bm{e}_t \in \mathbb{R}^d$.  We denote the sequence of embedding vectors of a query with $ \bm{x} = (\bm{x}_1, ...,\bm{x}_n )$.
%In  the neural network models,  each query is  a sequence of $T$ tokens,  with  $\textbf{x}_t \in \mathbb{R}^d$.  
 The network in Figure~\ref{fig:rnn} reads the input sequence one token at a time. At every time step $t$ a hidden state  $\bm{h}_t \in \mathbb{R}^d$ is produced   using the  recurrent equation 
\begin{align*}
\bm{h}_t &= f(\bm{W} \bm{x}_t  + \bm{U}  \bm{h}_{t-1} + \bm{b}) 
%\bm{o}_t &= \bm{W}_{s} \bm{h}_{t} + \bm{b} 
\end{align*}
where    $\bm{x}_t \in \mathbb{R}^k$  is the input token at time $t$ encoded as a vector,   $\bm{h}_{t-1} \in \mathbb{R}^d$ is the hidden state at time $t-1$, %$\bm{W}$ and $\bm{U}$ are input-to-hidden, hidden-to-hidden  weight matrices,
The parameters include  weight matrices $\bm{W}$  and $\bm{U}$, and a bias vector $\bm{b}$. $f(.)$ is a point-wise non-linear activation function, such as the Sigmoid or Rectified Linear unit (Relu)~\cite{Goodfellow-et-al-2016}. 
%LSTMs are a variant of RNNs, which address the long-term dependency issue in RNNs.  These models augment the RNN with a memory cell $c_t$

%Recurrent neural networks (RNNs) are a neural network model  that can process sequential data. 
%An RNN reads the input sequence one token at a time. At every time step, an output,  or hidden state, is produced. 





Standard RNNs suffer from  the \textit{vanishing gradient} problem.
In particular, during training, the gradient vector can grow or decay exponentially~\cite{tai2015improved,Goodfellow-et-al-2016}.
LSTMs are a more effective variant of RNNs. They are equipped with a memory cell, which helps  preserve the long-term dependencies better than standard RNNs. We describe the LSTM version from~\cite{zaremba2014learning}. %Figure~\ref{fig:lstmcell} shows a single LSTM Cell. 
The mathematical formulation  for the LSTM is as follows: 
\begin{align*}
\bm{\tilde{c}}_t &= \tanh(\bm{W}_c \bm{x}_t + \bm{U}_c \bm{h}_{t-1} + \bm{b}_c) \\
\bm{\Gamma}_u &= \sigma (\bm{W}_u \bm{x}_t +  \bm{U}_u \bm{h}_{t-1} + \bm{b}_u) \\
\bm{\Gamma}_f &= \sigma (\bm{W}_f \bm{x}_t +  \bm{U}_f \bm{h}_{t-1} + \bm{b}_f) \\
\bm{\Gamma}_o &= \sigma (\bm{W}_o \bm{x}_t +  \bm{U}_o \bm{h}_{t-1} + \bm{b}_o) \\
\bm{c}_t &= \bm{\Gamma}_u \odot \bm{\tilde{c}}_t + \bm{\Gamma}_f \odot \bm{c}_{t-1}\\
\bm{h}_t &= \bm{\Gamma}_o \odot \tanh(\bm{c}_t) 
\end{align*}
where $\odot$ is element-wise multiplication. The LSTM parameters are $\bm{W}_c$, $\bm{W}_u$, $\bm{W}_f$, $\bm{W}_o, \bm{U}_c$, $\bm{U}_u$, $\bm{U}_f$, $\bm{U}_o$ that are weight matrices, and   $\bm{b}_c$, $\bm{b}_u$, $\bm{b}_f$, $\bm{b}_o$ that are biases.   % $x_t \in \mathbb{R}^k$  is the current input at time $t$,  $\bm{h}_{t-1} \in \mathbb{R}^d$  and $\bm{h}_t \in \mathbb{R}^d$ are the hidden state at time $t-1$ and $t$. 
The memory cell $\bm{c}_t \in \mathbb{R}^d$  helps  model the long-term dependencies.  The gates $\bm{\Gamma}_i, \bm{\Gamma}_f,\bm{\Gamma}_o,\bm{\tilde{c}}_t \in \mathbb{R}^d$ help control the flow of information~\cite{Goodfellow-et-al-2016}.
We  use a three-layered LSTM model (shown in Figure~\ref{fig:threelayerlstm}).

\iffalse
\begin{figure}[htb]
\centering
	\subfloat[LSTM cell]
		{
		\includegraphics[width=0.5\linewidth]{architecture/lstmCell}
		\label{fig:lstmcell} 
		}
    	\subfloat[3-layer LSTM model]
		{
		%\includegraphics[width=0.3\textwidth]{architecture/gru-lstm-2-layer.pdf}
		\includegraphics[width=0.5\linewidth]{architecture/rnn_3.pdf}
		\label{fig:threelayerlstm} 
	}   
\caption{Using LSTM to make prediction}
\end{figure}
\fi

\begin{figure}
\centering
%\includegraphics[width=0.3\textwidth]{architecture/gru-lstm-2-layer.pdf}
\iffullpaperComposition
\includegraphics[width=0.7\textwidth]{architecture/rnn_3.pdf}
\else
\includegraphics[width=0.6\linewidth]{architecture/rnn_3.pdf}
\fi 
\caption{3-layer LSTM model. Here $\bm{h}_{t}^{l}$ denotes the hidden state of an LSTM in layer $l$ at time $t$.  At each time step,  $\bm{h}_{t}^{l}$  is fed as input to layer $l+1$. This allows the higher layers to capture more abstract concepts and longer term-dependencies. }
\label{fig:threelayerlstm} 
\end{figure}

\subsection{CNN}
\label{subsec:dbrec-cnn}


\iffalse
an input matrix $\bm{I} \in \mathrm{R}$ using a matrix of weights $\bm{K} \in \mathrm{R}^{m*n}$, referred to as the \textit{kernel}.
\begin{align*}
s[i,j] = (I*K)(i,j) & =  \sum_m \sum_n k(m,n) I(i-m,j-n)
\end{align*} 

\begin{align*}
s[i,j] = (I*K)(i,j) & =  \sum_m \sum_n k(m,n) I(i-m,j-n)
\end{align*} 
\fi


Convolutional Neural Networks (CNNs) %are a type of feed-forward neural network that have convolution layers interleaved with pooling layers~\cite{Goodfellow-et-al-2016}. 
are  feed-forward neural network models that can   process data which has grid-like topology, e.g., a sequence of concatenated token  vectors. 
 Their application in NLP, enables the model to extract the most important n-gram features from the input and create a semantic representation.  As a result,  long-term dependencies may not be preserved and  token order information is preserved locally.  CNNs however,  are known  to have comparable performance to RNNs,  they are faster and easier to train, and  are also parallelizable~\cite{young2018recent,bai2018empirical,yin2017comparative}. 

% \textcolor{red}{CNNS learn translation-invariant features,} and

Each layer in a CNN consists of  three stages~\cite{Goodfellow-et-al-2016}: convolution stage, detection stage, and pooling stage. We explain each of stages based on a 1-dimensional convolution operation, although higher dimensions are also possible. 

The \textbf{convolution stage} applies several  convolution operations.  In machine learning applications, a  convolution operator has two operands: a multidimensional array of weights, called the \textit{kernel}, and  a multidimensional array of input data. Convolving the input with the  kernel consists of sliding the kernel over all possible windows of the input. At every position $j$,  a linear activation $p_j$ is obtained by  %corresponding entries of the kernel and input are multiplied and the result is summed
computing  the dot product between the kernel entries and local regions of the input.   

\begin{figure}[ht]
\centering
       \includegraphics[width=1\linewidth]{architecture/convOp-1d-correct}
\caption{1D convolution operation. Here, $\bm{x}$ is the input, $\bm{w}$ is the kernel, and $\bm{x*w}$ is the output. Each element in $\bm{x*w}$ is produced by sliding the kernel over the input, and computing the dot product.}
\label{fig:cnn-op} 
\end{figure}


Figure~\ref{fig:cnn-op} shows an example of a 1-dimensional convolution operation. Let $\oplus$ denote the concatenation operation, and $\bm{x}_{1:n} = \bm{x}_{1} \oplus \bm{x}_{2} \oplus \dots \oplus \bm{x}_{n}$ denote the concatenated tokens in the query (stacked length-wise as a long column).   Let  $\textbf{x}_{j:j+k-1}$ represent a window of $k$ words, and $\bm{w} \in \mathbb{R}^{kd}$ denote a kernel. The dot product of $\bm{w}$ and each k-gram in the sequence is computed to obtain
%$a_i= (f*g)(i) & =  \sum_{j=1}^{m}  g(j).f(i-j + m/2)$
%where the kernel is $g$ and has length $m$, the input vector is $f$ with length $n$.  

%Generally, a 1d discrete convolution is obtained socher
%$a_n= (f*g)[n] & =  \sum_{j=1}^{-m}^{m}  f[n-m].g[m]$
\begin{align}
p_j = \bm{w}^{T} \bm{x}_{j:j+k-1} +b
  \end{align}
where  $b \in \mathbb{R}$ is a bias term. By sliding the kernel over all possible windows of the input, we obtain a sequence $\bm{p} \in \mathbb{R}^ {n-k+1}$.  Note, in the convolution stage, several kernels with varying window sizes   may be convolved with the data to produce different linear sequences. 


\begin{figure}[t]
\centering
       \includegraphics[width=1\linewidth]{architecture/cnn2_better.pdf}
\caption{1-layer CNN, adapted from~\protect\cite{kim2014convolutional}.}	
	%\caption[Architecture of a traditional convolutional neural network.]{The architecture of the original convolutional neural network, as introduced by LeCun et al. (1989), alternates between convolutional layers including hyperbolic tangent non-linearities and subsampling layers. In this illustration, the convolutional layers already include non-linearities and, thus, a convolutional layer actually represents two layers. The feature maps of the final subsampling layer are then fed into the actual classifier consisting of an arbitrary number of fully connected layers. The output layer usually uses softmax activation functions.}
	\label{fig:traditional-convolutional-network}
\label{fig:cnn} 
\end{figure}

In the \textbf{detector stage}, the linear sequence $\bm{p}$ is run through a non-linear activation function. This results  in a sequence of non-linear activations called  the  activation map
 \begin{align}
 \bm{a} = f(\bm{p})
  \end{align}
where $\bm{a} \in \mathbb{R}^{n-k+1}$,  and $f(.)$ is a non-linear activation function, e.g., Relu.
 
In the \textbf{pooling stage}  a pooling operation is applied to the activation map to summarize its   values. For example,  the max-pooling function  returns the maximum, i.e.,~ $g = \max\{\bm{a}\}$. Pooling  is used for down-sampling and reducing the size of the representation and building invariance to small transformations. In NLP and text applications, pooling also enables the model to handle inputs of varying size. 




%   Overall, each layer in a CNN acts as a feature detector that detects certain n-grams in the input. The main parameters of this layer are the kernel weights.
%The model consists of one convolution layer followed by a max pooling layer over time. This is followed by a fully connected layer and dropout. 
An example shallow CNN architecture~\cite{kim2014convolutional}. This network is shown in Figure~\ref{fig:cnn}. It consists of  a single  layer. In the convolution stage, several filters of  varying window size, $k \in \{3,4,5\}$, are applied and the resulting sequence is passed through a Relu function.  Different size sequence inputs and kernels result in  activation maps of different sizes. To deal with variable length of the input, and also obtain the most important feature, a max pooling operation is applied to obtain a single feature  per kernel, $g = \max\{\bm{a}\}$. The resulting features for all kernels are concatenated to produce a fixed size vector $\bm{g} \in \mathbb{R}^{K}$, where $K$ is the number of kernels.  This output is then used to create a fully connected layer, followed by a dropout layer. 

%\section{Application of NLP Models for Database Usability Problems}




\subsection{Prediction and training}
%Having defined models for  obtaining vector representations of the query, we   now proceed to defining an objective function for training the parameters of a representations and the  prediction model. We now describe how the above models are used to solve our usability problems.
Having obtained a vector representation for each query, we need to learn the mapping from the vector to the query property, e.g.,~ answer size.  In the prediction stage,  for the regression problems we  pass this vector through a linear unit 
\begin{align*}
\hat{y} &=  \bm{W}_{r} \bm{h} + \bm{b}_r   %\label{eq:rnn_prediction}
\end{align*}
where   $\bm{W}_{r}$  and   $\bm{b}_r$ are the prediction model weight and bias parameters  that should be learned.
In classification problems, we pass $\bm{h}$ through a softmax layer, to produce the predicted target value 
\begin{align*}
\hat{\bm{y}} &=  \textup{softmax} (\bm{W}_{s} \bm{h} + \bm{b}_s ) %\label{eq:rnn_prediction}
\end{align*} %and an output $\bm{o}_t \in \mathbb{R}^m$  are
where $\bm{W}_{s}$  and   $\bm{b}_s$ are     parameters   that the  model  must learn. The softmax function is $\textup{softmax} (\bm{z})_i = \frac{ \exp(z_i)}{\sum_j^n \exp{z_j} } $. 

Note, for three-layered LSTM $\bm{h} = \bm{h}_{n}^3$. For the CNN architecture, we also apply dropout and use $\bm{h} = (\bm{v} \circ \bm{g} )$. Here,  $\bm{v} \in \mathbb{R}^K$ is  a masking vector  of $K$ Bernoulli random variables with probability $p$ of being 1, and $\circ$ is element-wise   multiplication. At train time,  $\bm{v}$   randomly masks  $\bm{g}$. Dropout  helps prevent co-adaptation of the feature detectors~\cite{hinton2012improving}. 
 
 \iffalse here for regression problems, we  predict  $\hat{y}$ 
\begin{align*}
\hat{y} &=   \bm{W}_{r} (\bm{v} \circ \bm{g} ) + \bm{b}_r   %\label{eq:cnn_prediction}
\end{align*}
where the model must learn  the additional parameters $\bm{W}_{r}$ and $\bm{b}_{r}$.

For classification problems, a softmax layer is used for the final prediction
\begin{align*}
\hat{\bm{y}} &=  \textup{softmax} ( \bm{W}_{s} (\bm{v} \circ \bm{g} ) + \bm{b}_s  ) %\label{eq:cnn_prediction}
\end{align*}
where the model must learn the parameters $\bm{W}_{s}$ and $\bm{b}_{s}$. 
\fi 

%\vspace{4mm}
%\noindent \textbf{Objective Functions for Training.}
%\subsection{Training}
%\label{subsec:dbrec-objFunc}
%The models in Sections~\ref{subsec:dbrec-lstm}-~\ref{subsec:dbrec-cnn}, define a vector representation of the query.
%To learn the mapping from the input vector to the properties of the queries, we use
%Having defined models for  obtaining vector representations of the query, we   now proceed to defining an objective function for training the parameters of a representations and the  prediction model. 
%In this section we define the objective function used for training the models.  
Next, we discuss the  objective functions  we used to train the   models and learn  the parameters.  In the regression problems, the goal to predict a real number for each query, which corresponds to either the answer size or CPU time. In Section~\ref{subsec:dbrec_label_analysis} we observed the answer time and CPU time distributions had  a large number of outliers. Therefore, for the regression problems we use the Huber loss function~\cite{huber1964robust}, that is a hybrid between $l_2$ for small residuals and $l_1$ for large residuals 
\begin{align}
J(\theta) & = \sum_{i=1}^m h (\hat{y}^{(i)}(\bm{x}^{(i)},\bm{\theta}) - y^{(i)}) \label{eq:dbrec_reg_loss} \\
h(r) &=  
\begin{cases}
0.5 r^2, &  |r| \leq \epsilon \\
|r| - 0.5, & |r| > \epsilon.
\end{cases} 
\end{align}
where $m$ is the number of instances (queries) in the train set,  $\bm{\theta}$ is the set of all parameters that the model must learn, and $\hat{y}^{(i)}_{c}(\bm{x}^{(i)},\bm{\theta})$ is the  predicted value, i.e., predicted CPU time for query $i$.
 
 For error classification and session type classification, we use the %weighted 
cross entropy objective function
\iffalse
\begin{align*}
J(\bm{\theta}) & = \frac{1}{m} \sum_{i=1}^m - w_{c} \log \hat{\bm{y}}^{(i)}_{c}(\bm{x}^{(i)},\bm{\theta}) 
\end{align*}
\fi
\begin{align}
J(\bm{\theta}) & = \frac{1}{m} \sum_{i=1}^m -  \log \hat{y}^{(i)}_{c}(\bm{x}^{(i)},\bm{\theta}) 
\label{eq:dbrec_class_loss}
\end{align}
%where $m$ is the number of instances (queries) in the train set,  $\bm{\theta}$ is the set of all parameters that the model must learn, %$\bf{w} \in \bm{R}^K$ is a weight vector,  and $K$ is the number of classes,
here $c$ is the label of the correct class for instance $i$, and $\hat{y}^{(i)}_{c}(\bm{x}^{(i)},\bm{\theta})$ is the probability of class $c$ for instance $i$.
 
 
Note that  while  the traditional models fix the query vector representation (e.g.,~using the model explained in Section~\ref{subsec:dbrec-ngram_TFIDF}), and only optimize the weights of the prediction model, the neural network  models jointly train the representation and the weights of the prediction model. This is captured in the set of parameters $\bm{\theta}$ that are learned for each model.
For optimizing the neural network models, we examined Adam and  Adamax~\cite{kingma2014adam}, and found the latter obtained better results. 

 %for the prediction tasks from Section~\ref{sec:dbrec_prelim}.  
%Note, while  the traditional models fix the query vector representation and only optimize the weights of the prediction model, the neural network  models jointly train the representation and the weights of the prediction model.


\iffalse
huber link from pytorch website
http://statweb.stanford.edu/~owen/reports/hhu.pdf

https://www.cs.ubc.ca/~schmidtm/Documents/2005_Notes_Lasso.pdf
https://www.unige.ch/math/folks/sardy/Papers/robustIEEE.pdf

\fi



==> modified-results/busy-rownumber-modified.tex <==
\median&-&-&0.0675&-&1.6357\\
\ctfidf&500000&500000&0.0668&500000&1.0400\\
\ccnn&159&16801&0.0471&16801&\HL{0.7517}\\
\clstm&159&1943401&0.0452&529651&0.7678\\
\wtfidf&500000&500000&0.0668&500000&1.0922\\
\wcnn&85942&8595101&\HL{0.0441}&8595101&0.8472\\
\wlstm&85942&10521701&0.0443&9107951&0.8256\\

==> modified-results/error-sel-short-v-modified.tex <==

\mfreq&-&-&0.5951&0.0000&0.9863&0.0000&0.9730\\
\ctfidf&500000&1500000&0.5860&0.7131&0.9888&0.0053&0.9778\\
\ccnn&159&17403&0.1106&\HL{0.7961}&\HL{0.9897}&0.1669&\HL{0.9797}\\
\clstm&159&1944003&0.0830&0.6922&0.9893&\HL{0.2206}&0.9786\\
\wtfidf&500000&1500000&0.5836&0.6546&0.9885&0.0620&0.9773\\
\wcnn&85942&8597953&0.1006&0.7441&0.9894&0.2006&0.9790\\
\wlstm&85942&10522303&\HL{0.0691}&0.6971&0.9887&0.0018&0.9776\\

==> reviews.tex <==
\section*{Reviews}

\blue{We are very grateful for the valuable and constructive comments provided by the meta-reviewer and reviewers to help improve this work. We have revised our submission accordingly to address all the comments; to correct presentation issues and clarify concepts. For your convenience, our responses, and new/changed text are highlighted in blue.}

\subsection*{Reviewer 3}

\blue{Thank you for reading our paper carefully and your comments. We have revised the paper as per your suggestions. Detailed comments are grouped alongside their corresponding Weak comment, when applicable.}

%\rItem{Questions:}  1. Overall evaluation: Weak Reject, %2. Reviewer's confidence: Some Familiarity, 3. Novelty: Medium, 4. Importance: SIGMOD attendees will learn something interesting from the paper.

%\rItem{5. Summary of contribution:} This paper describes how to formulate efficient SQL queries without any statistics from the database and the query execution plans. The paper adapts data-driven machine learning models that rely on large query workloads to solve four problems (predicting the error class, CPU time, answer size, and prediction class) that help both end users and DBAs by providing query insights. Based on comprehensive analysis of two real-world query workloads (SDSS and SQLShare), experiments show the LSTM and CNN neural network architectures outperformed more traditional machine learning models and more simple baselines. While the paper solves an interesting problem, it can also be improved by providing more details on why its methods work well and better organizing the paper.

%\rItem{6. List strong points:} S1: Solves the interesting problem of using machine learning to predict four outcomes of a query and thus help facilitate query composition. S2: Provides insightful analyses on two important workloads: SDSS and SQLShare. S3: The experimental results are promising.

%\rItem{List weak points:}

\rItem{W1:} The proposed methods should be more generalized where there is some intuition on when some machine learning models work better than others. 

\nfeedback{  We thank the reviewer for this comment. We have included a discussion  in our list of contributions in Section~\ref{sec:dbrec-introduction}, and in the highlighted sentences in   Sections~\ref{sec:discussion_model} and~\ref{sec:discussion_qualitative}. Briefly, our results indicate that neural network character-level models, e.g., \ccnn and \clstm, perform better under various settings and as the complexity of the queries grow. This is intuitively because they learn features (as opposed to being limited to a pre-determined set of features) in the workloads, which subsequently   helps them better predict. \ccnn outperforms \clstm in different problems because \clstm is sequential and sensitive to the query length, whereas \ccnn focuses on learning local features (so it is locally sequential and less sensitive to length).}%\mostafa{I think we need more detailed explanation in Section~\ref{sec:dbrec_emp_eval}.}\footnote{RAP: I agree. I'm not at all convinced that the reviewer is going to be satisfied with a brief paragraph}

\rItem{W2:} The experiments need to include error analyses of the models and comparisons with manual cost models.

\nfeedback{ Thank you for this comment. We note the following: 
(1) We added a new error analysis based on qerror of the models in Table~\ref{tab:qerror}.   Please see our response to D5. 
(2) For manual cost models, we added (\opt) which  is a linear regression model that predicts the CPU time from query optimizer cost estimates~\cite{li2012robust,ganapathi2009predicting,akdere2012learning} .  Please see highlighted section in the  ``Methods'' subsection in ~\ref{sec:dbrec_exp_setup} and the corresponding empirical analysis in 6.2.2 and 6.2.3. Generally, our results are similar to the past work:  we found the query optimizer is not very precise for CPU time estimations.  This may be due to the fact that the query optimizer cost model assumes I/O is the most time-consuming and so its  cost estimates are  mostly correlated with I/O, whereas several time-consuming queries (like aggregates over numeric types)  are performed in memory. Another reason might be that the linear regression model is insufficient, and  we may need a non-linear model which maps the cost estimates to CPU time estimates. This might lead to  performance improvements in \settingThree, 
(3) We continue to provide in this draft the error analysis that we had in the previous draft: we report  Huber loss and mean square error for test set in regression problems (e.g., Table~\ref{tab:sqlshare_busy_prediction_results_sel}  and Figure~\ref{fig:mse_by_properties_busy}). For classification problems we report  Cross-Entropy loss of the test set and accuracy of the models (e.g., Table~\ref{tab:error_prediction_results_sel}). 
}

%\nfeedback{We report three different errors that evaluate our models from different perspectives: Huber loss which evaluates our models performance, MSE and q-error which can help us determine how well the models perform in our application of facilitating query composition. TODO: For answer size prediction, which is a common problem in the literature, we compare the performance of our models with the existing manual cost models.\mostafa{We have Huber loss and MSE and we should only add some analysis of q-error.}.}

%\feedback{Our error analysis is reported in sections 6.2 and 6.3. The quantitative results in Tables 1-4 report error values for the test set (denoted by ``loss'') and accuracy measurements (f-measure and accuracy). Additionally, our qualitative analysis in Section 6.3 also reports Mean Square Error (MSE) for the regression problems (Figure 9). However, we will change the presentation of the material to resolve the ambiguity.}

\rItem{W3:} There needs to be more discussion on how to perform well in the homogeneous schema and heterogeneous schema cases.

\rItem{D4:} In Sections 6.2.2-6.2.3, the coverage of the homogeneous schema and heterogeneous schema cases is rather thin and can be improved. In particular, there needs to be a discussion on how to improve the current proposed methods to work better in such challenging settings.

\nfeedback{(W3 and D4)  We acknowledge that this is an important issue and needs more discussion. In this work we took the first steps to compare several models in our heterogeneous settings. We showed character-level CNNs are able to generalize better compared to traditional and word-level models and under the \settingTwo and \settingThree query facilitation problem settings. Our next step is to apply ideas for transfer-learning in neural networks to improve the performance of \ccnn in our heterogeneous settings. We mention this in the blue sentence in the last paragraph of Section~\ref{sec:dbrec-conclusion}.}

\rItem{W4:} The presentation of the paper can be improved. 

\rItem{D6:} Throughout the paper, the presentation can be improved. The Introduction seems to contain unnecessary details (especially the last paragraph before the summary) while being vague about the exact problem being solved. The details on SDSS seems scattered in Section 2 up to Section 6, so it is difficult to get a coherent picture. Instead, it would be better to move all the workload-specific details into Section 6. Also, experimental results frequently appear before Section 6 (e.g., last paragraph of Section 4.3), and it is difficult to keep track of them.

\nfeedback{(W4 and D6)  We agree that the raised issues hinder the paper's readability and we applied the following to resolve them: 
(1) We added "Workload Analysis Implications" (Section~\ref{subsec:dbrec_analysis_implications}) which explains how the workload analysis relates to model selection  (Section~\ref{subsec:dbrec_analysis_implications_model_selection}) and model evaluation (Section~\ref{subsec:dbrec_statement_complexity}). 
(2) We moved "Workloads and Analysis" (Section~\ref{sec:dbrec_dataset_and_analysis}) to before "Methods" (Section~\ref{sec:dbrec_methods} which used to be Section~4) since the analysis in Section~\ref{subsec:dbrec_analysis} is prerequisite for our discussion in Section~\ref{sec:dbrec_methods}. 
(3) We moved discussion on SDSS in the beginning of Section~\ref{sec:dbrec_motivation} to Section~\ref{sec:dbrec_dataset_and_analysis}.
%TODO: Adding q-error analysis in Section~\ref{sec:results}?
(4) We moved the last paragraph of the introduction which was about model selection to Section~\ref{subsec:dbrec_analysis_implications}. (5) We updated the introduction to clarify the problems by explaining heterogeneous vs homogeneous settings (the third paragraph in the second page).\ignore{ (7) TODO:checking sentences about our results before section 6 (last paragraph in Sec 4.3 that we can move to Sec 6, at least part of it).}}

\rItem{D1:} The paper applies 6 machine learning models on the two workloads without enough insight on why they should work well. For example, CNNs are known to work well in computer vision problems, so why should they work the best on SQL queries? In addition to the models, a critical factor in prediction accuracy is the data distribution. In the evaluations, how much does data distribution influence accuracy versus the model architecture? It could be that, for SQL sources other than SDSS and SQLShare, models other than LSTM and CNN perform the best. At the least, there should be some general guidelines on how to choose models.

\nfeedback{The reviewer raises three important questions in this comment. We briefly answered the first question in our response to the reviewer's W1. About the second question, we empirically show both model and data distribution greatly impact our predictions. For data distribution, we study different problem settings for which the data distribution can change from training to test (Section~\ref{sec:results}). With respect to the distribution of the queries in the workload and their labels, we extensively study them in Sections~\ref{subsec:dbrec_statement_analysis} and \ref{subsec:dbrec_label_analysis} and we run experiments for different data distributions in Sections~\ref{sec:dbrec_performance_by_session_class} and~\ref{sec:perfstr}. For the last question, we discuss our model selection in Section~\ref{subsec:dbrec_analysis_implications_model_selection}. Our results show that although traditional and simple models sometimes slightly outperform modern neural networks for simple queries in homogeneous settings, character-level CNN performs better across different settings and for complex queries.\ignore{
Note, our empirical results also confirm our intuitions. 
Explaining (both in Intro and in Experiments) why CCNN outperforms other models. 1.1- Why clevel models perform better? 1.2- Why Shallow CNN outperforms LSTM and Traditional models?}}

\ignore{\st {Although we have implicitly discussed the intuitions for choosing the models (in the introduction, Section 4, and beginning of Section 7), we agree with the reviewer that we should explain the intuitions more clearly (in Section 4). As a starting point, we wanted to include a broad set of architectures that apply to SQL queries, ranging from the traditional models to deep learning models. There are several options in the deep learning literature, but we wanted to include models that are successful in similar domains, for similar problems. CNNs and recurrent neural networks (RNNs) are the dominant models in NLP. Specifically, RNNs can treat SQL queries as sequential inputs, and we chose LSTMs from this group. On the other hand, CNNs are feed-forward NNs that can automatically identify n-grams. CNNs have recently been shown to provide competitive results with several more sophisticated architectures and are easier to train and interpret[3,28,51,52,53]. Based on these intuitions we selected the models, and analyzed them at the word level and character level.}}

\rItem{D2:} In Figure 1, the impression is that Query (b) should be avoided because it takes too long. What if that is the correct behavior, and the user is supposed to wait for the desired results? Making query composition decisions seems much more complex than simply looking at the CPU time and comparing it with a threshold.

\nfeedback{The user should avoid the query because it might call {\tt dbo.fPhotoFlags('BLENDED')} many times for different records. The user can rewrite the query to call the function only once since it returns the same answer for every record. We updated the first paragraph in Section~\ref{sec:dbrec_motivation} to clarify this issue. Note that we facilitate query composition by predicting properties of such a query, e.g., its CPU time, prior to execution. This can hint to the user to check the query when the properties are unexpected, e.g., the CPU time of a query is unexpectedly high. Identifying inefficient queries and suggesting rewriting for the queries are beyond the scope of this paper.}

\rItem{D3:} Section 5 comes out of the blue, and it is not clear what are the takaways from analyzing the SDSS and SQLShare workloads. How does this analysis relate to the proposed methods? For example, does the analysis help identify the important features for the machine learning models?

\nfeedback{ We apologize for the confusion, and we agree that this should be clarified. This section is an essential part of the paper and helps in both selecting proper models and evaluation methods. Please see our response to W4, where we have elaborated on this issue.}

%\feedback{We appreciate this comment and will re-write to resolve the presentation issue. We needed the workload analysis to examine the prediction tasks and model performance more thoroughly. Our qualitative analysis of the prediction models in Section 6.3 relies on the workload analysis and query structural properties.}


\rItem{D5:} In Section 6, it is difficult to fully understand the results just by looking at performance properties. Instead, there needs to be an analysis of what query property predictions succeed and fail. For example, suppose there are two textually similar queries Q1 and Q2, but their results are vastly different because of the data distribution. Would the LSTM and CNN models still make the correct predictions? If not, why? In addition, there needs to be comparisons with manual cost models instead of stating that they may be imprecise.

\nfeedback{ We added more analysis of our answer size prediction in SDSS and in \settingOne (see the highlighted paragraph in Section~\ref{sec:results_setting1}). We use qerror, which shows the factor by which an estimate differs from the true answer size. For example, if $8$ and $2$ are subsequently estimated and actual answer sizes, qerror is $4$. Our results in Table~\ref{tab:qerror} show that \ccnn and \clstm can estimate answer size of $85\%$ of the queries in the experiment with an acceptable qerror of $6.79$. We also analyze qerror of CPU time prediction for SQLShare and in \settingTwo and \settingThree (see Sections~\ref{sec:results_setting2} and~\ref{sec:results_setting3}). With regards to specific queries, we investigate different properties of two queries in Figure~\ref{fig:q1} and~\ref{fig:q2} in our case study in Section~\ref{sec:dbrec_qualatative_analysis}.}

%\nfeedback{TODO: see R3.W2 (the first item) and W3.D1.}


\rItem{Required changes for a revision:} R1: Please address Reviewer 3 W2, Reviewer 3 D1, and Reviewer 3 D3 in the author response.


\subsection*{Reviewer 6}
\blue{Thank you for reading our paper carefully and your insightful comments.}
%\rItem{Questions} Overall evaluation: Accept % 2. Reviewer's confidence Expert 3. Novelty Medium 4. Importance: select all that apply: The paper is likely to influence other research in the community The paper contains controversial ideas and/or will generate interesting discussion SIGMOD attendees will learn something interesting from the paper

%5. Summary of contribution (in a few sentences) The authors analyze query workloads to make predictions about size, runtime, and error prediction, as well as classifying queries by client category. Several methods are evaluated, and some clear insights emerge about the architecture of the NNs one should use.

%6. List 3 or more strong points, labeled S1, S2, S3, etc. S1 Improved workload analysis over prior work S2 An important area that is underrepresented in the literature S3 Rigorous experiments
%\rItem{List of weak points}

\rItem{W1:} No direct comparison of experimental results with prior work
%We have added  a  new model (opt) that is based on the cost  estimates of the query optimizer. 

\nfeedback{ For manual cost models, we added (\opt) which  is a linear regression model that predicts the CPU time from query optimizer cost estimates~\cite{li2012robust,ganapathi2009predicting,akdere2012learning} .  Please see highlighted section in the  ``Methods'' subsection in ~\ref{sec:dbrec_exp_setup} and the corresponding empirical analysis in 6.2.2 and 6.2.3. Generally, our results are similar to the past work:  we found the query optimizer is not very precise for CPU time estimations.  This may be due to the fact that the query optimizer cost model assumes I/O is the most time-consuming and so its  cost estimates are  mostly correlated with I/O, whereas several time-consuming queries (like aggregates over numeric types)  are performed in memory. Another reason might be that the linear regression model is insufficient, and  we may need a non-linear model which maps the cost estimates to CPU time estimates. This might lead to  performance improvements in \settingThree, 
(3) We continue to provide in this draft the }

\rItem{W2:} Some unsubstantiated claims of novelty; the motivation has been clearly articulated in cited papers

\nfeedback{ Our main contributions are (1) using query performance prediction for the application of facilitating query composition, (2) an extensive analysis of two public large-scale workloads for model selection and model evaluation, (3) comparing a broad set of data-driven models for these prediction problems. We updated our list of contributions at the end of the introduction to clarify this. We acknowledge that applying data-driven models with large-scale workloads for query properties prediction are first discussed in~\cite{jain2018query2vec,jain2018database},  and we have provided a   paragraph in Section~\ref{sec:dbrec-introduction} where we point out our differences.}

\rItem{W3:} The title and target of the paper are unfocused.

\nfeedback{ We address four query property prediction problems that can facilitate SQL query composition, which is the main application of this work. The title of the paper highlights this application and our extensive analysis of the workloads.\ignore{ \red{TODO: He/she has a point! Analysis does not sound related to facilitating query composition.}}}

\rItem{D1:} It's not clear that the paper actually provides evidence of facilitating SQL composition.

\nfeedback{Our results indicate that we can estimate several properties of SQL queries prior to their execution which is the first step towards our goal to facilitate query composition. We provided additional analysis using qerror to support this claim (see the last paragraph in Section~\ref{sec:results_setting1}). Our next steps are to design, implement, and evaluate a query composition facilitation system using models to help users write queries. We intend to conduct a user-centric study in another work.}

\rItem{D2:} The query prediction problems in Section 3 are very similar to those described in Query2Vec (Jain 19).

\nfeedback{We acknowledge that some  problems have separately been defined in the literature for different applications. We added a paragraph in the introduction for Query2Vec (Jain 19)  [22,24]. % Please see the footnote before Definition~\ref{df:problems}.
}

\rItem{D3:} It's not clear that the notation is needed; the prediction problems are straightforward.

\nfeedback{ We agree with the reviewer and we updated Definition~\ref{df:problems}.}

\rItem{D4:} There seem to be two papers here: one is a workload characterization paper, the other is a set of prediction tasks. I think the paper would benefit from a more focused approach.

\nfeedback{ Thank you for this comment which helped us better clarify our ideas.  To resolve the issue, we added "Workload Analysis Implications" (Section~\ref{subsec:dbrec_analysis_implications}) which explains how the workload analysis relates to model selection  (Section~\ref{subsec:dbrec_analysis_implications_model_selection}) and model evaluation (Section~\ref{subsec:dbrec_statement_complexity}). In addition, because "Workloads and Analysis" in Section~\ref{sec:dbrec_dataset_and_analysis} is a prerequisite for model selection in Section~\ref{sec:dbrec_methods}, we swapped their order in the new version.%. So"Workloads and Analysis" (Section~\ref{sec:dbrec_dataset_and_analysis}) to before "Methods" (Section~\ref{sec:dbrec_methods} which used to be Section~4) .
}


\rItem{D5:} The paper is somewhat incremental over [19] and [20], though the treatment is very thorough, and the methods are more advanced and the results appear better.

\nfeedback{We acknowledge that ours is not the first work that considers data-driven models with large-scale workloads. We added a new paragraph in Section~\ref{sec:dbrec-introduction} to briefly compare with the leading work in this area (\cite{jain2018query2vec,jain2018database} that are [19,20] in our first submission). We thank the reviewer for recognizing our effort for studying several data-driven models with large-scale workloads.}

\rItem{D6:} The effect of literals in the queries is not studied. Removing literals and retaining literals can have an effect on performance for heterogeneous cases.

\nfeedback{As stated in Section~\ref{subsec:dbrec_analysis_implications}, we examine the effect of literals via the character-level models (where literals are retained). We only replace the literals with special tokens for the word-level models. We plan to study extensions of models with word-level representation for literals (e.g. categorizing numerical literals).}

\subsection*{Reviewer 8}

\blue{Thank you for your insightful comments to improve this work. We outline the corresponding changes below.}

%\rItem{Questions:} 1. Overall evaluation Weak Accept% 2. Reviewer's confidence Some Familiarity 3. Novelty Medium 4. Importance: select all that apply: SIGMOD attendees will learn something interesting from the paper

%5. Summary of contribution (in a few sentences) In this paper, the authors propose to use machine learning (ML) techniques to address the problem of facilitating SQL query composition and analysis. The solution framework relies on exploring existing, publicly available query workloads. For the solution implementation, the authors develop three different ML-based models: a traditional model based on classic feature engineering methods like TFIDF, and two models built on Deep Learning (DL). The authors design and conduct a set of analysis and experiments to support their assumptions and findings.

%List 3 or more strong points, labeled S1, S2, S3, etc. S1: the problem that the authors try to address is interesting and important S2: the authors explore DL methods to solve the problem S3: the authors conduct extensive evaluation and analysis 

%\rItem{List of weak points:}

\rItem{W1 and D1:} W1: some assumptions made in the paper are too strong and not justified (see D1). D1: The authors claim that the access to the database instance can be infeasible, therefore focus on extracting useful knowledge from the database workload. However, it is not clear whether the workload will be available for use for many real-world problems. The authors should point out that (a) some real applications where database workloads are accessible other than SDSS and SQLShare, or (b) the knowledge learned from SDSS or SQLShare are transferable to facilitate queries in other database domains (see D2).

\nfeedback{ We appreciate this important comment about the applicability of our solutions. We consider models for both scenarios in (a) and (b). For (a), there are publicly available scientific and academic workloads (e.g. SDSS and SQLShare) and private workloads (e.g. Snowflake) owned by large companies. (Please see the first paragraph in page 2.) For (b), we study different problem settings where query workload and the given query are from different databases (see the second paragraph in page 2). We formalize these scenarios in Definition~\ref{df:settings} and study them in our experiments in Section~\ref{sec:results}.}

\rItem{W2 and D2:} W2: it is not clear whether the model learned on one workload dataset can be transferable to other DB queries (see D2). D2: The definition of the problem is vague. The authors should clearly define the problem and the application setting. For example, given a database X, (a) is the problem to use workload of X to facilitate future queries on X? Or (b) is the problem to learn from some publicly available workload resources to extract universal knowledge, and facilitate future queries on X?
If it is the former case, there will be some limitation of the proposed solution, as it is not guaranteed such workload is available. If it is the latter one, the authors should emphasize on the fact that the knowledge learned is transferable, and back up with more detailed evaluation in the experiment section. The definition 4 in the paper is good, but still a bit vague to me.

\nfeedback{Thank you for raising this concern which helped us clarify the problem settings our work addresses. As we mentioned in our response to W1 and D1, we added Definition~\ref{df:settings} that specifies three problems settings and captures both (a) and (b). The scenario in (a) is \settingOne where $\mc{W}$ and $Q_*$ are over the same database instance. The scenario in (b) is represented by \settingTwo and \settingThree. We explain in the new paragraph after the definition that there are other possible settings depending on the queries execution conditions. We show in our experiments in Section~\ref{sec:results} that the knowledge learnt from a workload over a database can be used for estimating query properties in a different database.}

%\feedback{We appreciate this comment. Although we have already considered the different settings the reviewer has mentioned, we will revise to make it clearer. In the paper, we refer to these different settings as homogeneous instance, homogeneous schema, and heterogeneous schema right after definition 4. We realize that we need to modify Definition 4 and include these various settings in it. The quantitative experiments related to various settings are in Section 6.2.1- 6.2.3, while the qualitative experiments related to various settings is in Section 6.3.3.}

\rItem{W3:} The novelty of the technical details is limited (see D3). 

\rItem{D3:} The novelty of the technical details is limited. The models used in the paper are well developed and used in CV and NLP for years.

\nfeedback{(W3 and D3) Our main technical contributions are (1) formalizing the property prediction problems for SQL queries in different settings in Section~\ref{sec:dbrec_problem_definition}, (2) applying different data-driven models for large-scale workloads considering the challenges we explained in Section~\ref{subsec:dbrec_analysis_implications}, (3) analysing large-scale workloads and extracting training and test data from such workloads.}

\rItem{D4:} The classification problems and the regression problems defined in Definition 4 are correlated. For example, if a query doesn't run and is classified as ``severe'', the query runtime and answer size will also be affected. It seems the in the proposed model, the classification and regression are performed separately. Does the model capture the correlation?

\nfeedback{ We did not consider possible correlations between the query labels in our performance prediction problems. We agree that considering these correlations could improve predictions, although that requires workloads with multiple labels which restricts the applicability of the models. We noted this in our future work (see the blue sentences in the last paragraph in Section~\ref{sec:dbrec-conclusion}).}

\rItem{D5:} I noticed that the classification accuracy is low for minor query types in Table 1. I wonder if any weighted loss has been applied for the model training. What is the design choice here for the loss function? Are different classes treated equally? Similarly, is there any weighting for the regression tasks in Table 2? Are queries with different runtime equally important?

\nfeedback{ Thank you for raising this concern. Please see Section~\ref{subsec:dbrec_analysis_implications_model_selection} where we explain how our workload analysis relates to the choice of model selection and train loss functions. }

%\feedback{\st{The reviewer has raised an important point, we will revise the paper to make it clearer. Currently, the design choice for the loss function of each model is explained (briefly) in Sections 4.1-4.3. As mentioned in the 2nd paragraph of the conclusion, the classification problems suffer from class imbalance. The choice of weights in the classification loss function is application dependent and should be determined w.r.t. classes of queries that are most important for that problem. For example, in session classification, we can train a model that detects bots with high accuracy, if that is what the domain requires. However, in the absence of such information, we used equal weight in our loss function. An interesting future direction is to address class-imbalance, but this requires additional intuitions or assumptions about the importance of query classes. A similar discussion applies for the regression problems.}}

==> sql_example_table.tex <==
\iffalse
%sqlID	181511768	
\begin{lstlisting}[
	language=SQL,
	caption=Query 1,
	captionpos=b,  
    basicstyle=\footnotesize,
    stepnumber=1,
    showstringspaces=false,
    tabsize=1,
    breaklines=true,
    breakatwhitespace=false,
    frame=single,
    label=lst:error_example_query]
select top 100 run,rerun,field,camcol,sky_r,skypsp 
from field;
\end{lstlisting}
\end{table}
%numbers=left,
%label=lst:error_example_query
\fi

\clearpage
\section{Additional SQL Query Examples}
%In Figure~\ref{fig:example_sql_queries_all}, we show examples from our collected dataset:



\begin{figure}[!htbp]
\iffalse
\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q1.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class is 0,  session class is BOT,  answer size is 1, and CPU time is 0.015] %&0& BOT & 1& 0.015\\%sqlID	168294239
{ \usebox{\mylistingbox}}
\fi


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q9.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class   0 session class BROWSER   answer size  847  cpu time 0.039999999 ]% & 0 & BROWSER & 847 & 0.039999999 \\%75345416
{ \usebox{\mylistingbox}}


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q2.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class  -1  session class noWebhit  answer size 0  cpu time 0] % &-1& noWebhit & 0 & 0\\%sqlID	116226135 statementID 53065814
{ \usebox{\mylistingbox}}


	
	
	


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q2-2.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[error class  -1  session class noWebhit  answer size 0  cpu time 0] %&-1& noWebhit & 0& 0  % sqlID 115897182 statementID 48306361
{ \usebox{\mylistingbox}}



  




\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q2-3.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  -1  session class noWebhit  answer size 0  cpu time 0] %&-1& noWebhit & 0& 0\\ sqlid 106144597 entered 5 times overall
{ \usebox{\mylistingbox}}





\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q2-4.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  -1  session class PROGRAM  answer size 0  cpu time 0] % &-1& PROGRAM & 0& 0\\%sqlid 116373895 invalid column name zconf
{ \usebox{\mylistingbox}}


\caption{Example SQL queries in SDSS workload.}
\label{fig:example_sql_queries_all}
\end{figure}


%\renewcommand{\thefigure}{\arabic{figure} (Cont.)}
%\addtocounter{figure}{-1}


\begin{figure}
\ContinuedFloat


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q2-5.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class  -1  session class noWebhit  answer size 0  cpu time 0] %&-1& noWebhit & 0& 0 %5642913	
{ \usebox{\mylistingbox}}








\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q2-6.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  -1  session class noWebhit  answer size 0  cpu time 0] %%116409556 passes syntax check but runs into error, "Invalid object name '#x'", errorMessageID is 16, errorMessage is error: must be a select statement:
{ \usebox{\mylistingbox}}







\iffalse

\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q2-7.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  -1  session class BROWSER  answer size 0  cpu time 0]%\\%116409573 passes syntax check but runs into error, "Invalid column name 'SpecClass'.", errorMessageID is 16, errorMessage is error: must be a select statement:
{ \usebox{\mylistingbox}}
\fi


\label{fig:example_sql_queries_all}
\caption[]{Example SQL queries in SDSS workload.}
%\phantomcaption
\end{figure}




\begin{figure}
\ContinuedFloat

\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q3.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class  1  session class noWebit  answer size 99999999  cpu time 0]%sqlID	181511768% not in test, fine	
{ \usebox{\mylistingbox}}





\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q4.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  0  session class PROGRAM   answer size 0   cpu time 0 ]%& 0 & PROGRAM& 0& 0\\ %11951038% not in test, fine	
{ \usebox{\mylistingbox}}





\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q5.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  0   session class PROGRAM  answer size 0   cpu time 0.035]% & 0 &PROGRAM &0& 0.035\\%101535576% not in test, fine	
{ \usebox{\mylistingbox}}






\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q6.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class 0 session class  BROWSER answer size 0   cpu time 1.388 ]% & 0 & BROWSER& 0 & 1.388\\ %46889771
{ \usebox{\mylistingbox}}





\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q7.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  0  session class noWebhit   answer size 0   cpu time  0]%& 0 & noWebhit &   0 & 0 \\ %174736798% not in test, fine	
{ \usebox{\mylistingbox}}






\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q8.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class  -1  session class BROWSER   answer size 0  cpu time 0]% & -1 & BROWSER & 0 & 0\\%103563657 error: limit is top 500000% not in test, fine	 %0 ->>> 0.6931
{ \usebox{\mylistingbox}}





\caption[]{Example SQL queries in SDSS workload.}
\label{fig:example_sql_queries_all}
%\phantomcaption
\end{figure}

\begin{figure}
\ContinuedFloat




\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q10.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class  0  session class PROGRAM   answer size   1521  cpu time  0.017999999 ]%& 0 & PROGRAM  & 1521 & 0.017999999\\%9882847
{ \usebox{\mylistingbox}}






\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q11.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class  0  session class BROWSER   answer size   26703014 cpu time  156.90601 ]%& 0 & BROWSER & 26703014 & 156.90601\\%5497473# runs into error for me
{ \usebox{\mylistingbox}}






\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q12.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  1  session class noWebhit   answer size   99999999 cpu time 0 ]% & 1 & noWebhit & 99999999 & 0\\%97832379
{ \usebox{\mylistingbox}}



\caption[]{Example SQL queries in SDSS workload.}
%\phantomcaption
\label{fig:example_sql_queries_all}
\end{figure}

\begin{figure}
\ContinuedFloat


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q13.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  0   session class noWebhit   answer size 99999999   cpu time  0] % & 0 & noWebhit & 99999999 & 0\\%81753190
{ \usebox{\mylistingbox}}







\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q14.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class  0  session class noWebhit   answer size 500000  cpu time 50.659 ]%& 0 & noWebhit & 500000 & 50.659\\%105258941
{ \usebox{\mylistingbox}}






\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q15.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class 0   session class  noWebhit answer size  99,999,999  cpu time 100,000,000 ]% & 0 & noWebhit & 99,999,999 & 100,000,000\\%109188307 error message ID is 2, error message is 0
{ \usebox{\mylistingbox}}


\caption[]{Example SQL queries in SDSS workload.}
%\phantomcaption
\label{fig:example_sql_queries_all}
\end{figure}

\begin{figure}
\ContinuedFloat

\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q16.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class   1 session class  noWebhit answer size  19  cpu time 0 ]% & 1 & noWebhit & 19 & 0\\%5226180
{ \usebox{\mylistingbox}}

\caption[]{Example SQL queries in SDSS workload.}
%\phantomcaption
\label{fig:example_sql_queries_all}
\end{figure}

\begin{figure}
\ContinuedFloat


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q17.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[  error class  1  session class BROWSER   answer size 147  cpu time 0]% & 1 & BROWSER & 147 & 0% not in test, fine	\\%94331925
{ \usebox{\mylistingbox}}






\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q18.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[ error class   1 session class noWebhit   answer size 4474  cpu time 0 ]% & 1 & noWebhit & 4474 & 0% not in test, fine	\\%79618208 seems good
{ \usebox{\mylistingbox}}



\caption[]{Example SQL queries in SDSS workload.}
%\phantomcaption
\label{fig:example_sql_queries_all}

\end{figure}











\iffalse
\begin{figure}


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q19.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[Q19  error class  0  session class BOT   answer size 5477142  cpu time  67.660001]
{ \usebox{\mylistingbox}}
% & 0 & BOT & 5477142 & 67.660001\\%5642177  busy is an average of [101.629, 33.691002]


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q20.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[Q20  error class 0   session class  noWebhit answer size 596   cpu time  0.0060000001 ]
{\usebox{\mylistingbox}}
% & 0 & noWebhit & 596 & 0.0060000001\\%173177393 two entries just the session class is noWebhit and BROWSER, rows is an average of [596, 596]%busy is an average of [0.0060000001, 0.0060000001]


\caption[]{Example SQL queries in SDSS workload.}
%\phantomcaption
\label{fig:example_sql_queries_all}

\end{figure}
\fi










\begin{figure}
\ContinuedFloat



\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q21short.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[Q21short  error class  0  session class noWebhit   answer size 298  cpu time  28.969 ]
{\usebox{\mylistingbox}}

% & 0 & noWebhit & 298 & 28.969 \\%97856791 



\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q22.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[Q22  error class 0   session class BROWSER   answer size   98877  cpu time 41.342999]
{ \usebox{\mylistingbox}}
%& 0 & BROWSER & 98877 & 41.342999 \\%105151025 
 
\caption[]{Example SQL queries in SDSS workload.}
% \phantomcaption
\label{fig:example_sql_queries_all}

\end{figure}

\begin{figure}
\ContinuedFloat


\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q23.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[Q23  error class  0  session class    BOT answer size  52723    cpu time  3.01]
{ \usebox{\mylistingbox}}
%& 0 & BOT & 52723 & 3.01\\%37983399



\begin{lrbox}{\mylistingbox}%
\begin{minipage}{1\linewidth}%
\lstinputlisting{SQL-Examples/Q24.txt}
\end{minipage}%
\end{lrbox}%
\subfloat[Q24  error class 0   session class  BOT  answer size 2367  cpu time 2.1600001]
{ \usebox{\mylistingbox}}
%& 0 & BOT & 2367 & 2.1600001\\%95286756

\caption[]{Example SQL queries in SDSS workload.}
%\phantomcaption
\label{fig:example_sql_queries_all}

\end{figure}


%\renewcommand{\thefigure}{\arabic{figure}}

